Learning Nearly Decomposable Value Functions Via Communication Minimization

Reinforcement learning encounters major challenges in multi-agent settings, such as scalability and non-stationarity. Recently, value function factorization learning emerges as a promising way to address these challenges in collaborative multi-agent systems. However, existing methods have been focusing on learning fully decentralized value functions, which are not efficient for tasks requiring communication. To address this limitation, this paper presents a novel framework for learning nearly decomposable Q-functions (NDQ) via communication minimization, with which agents act on their own most of the time but occasionally send messages to other agents in order for effective coordination. This framework hybridizes value function factorization learning and communication learning by introducing two information-theoretic regularizers. These regularizers are maximizing mutual information between agents' action selection and communication messages while minimizing the entropy of messages between agents. We show how to optimize these regularizers in a way that is easily integrated with existing value function factorization methods such as QMIX. Finally, we demonstrate that, on the StarCraft unit micromanagement benchmark, our framework significantly outperforms baseline methods and allows us to cut off more than $80\%$ of communication without sacrificing the performance. The videos of our experiments are available at https://sites.google.com/view/ndq.

==> 4-Method.tex <==
\section{Methodoloty}\label{sec:algorithm}
In this section, we propose to learn nearly decomposable value functions with communication, a new framework to overcome the miscoordination issue of full factorization methods. Our framework adopts the centralized training and decentralized execution paradigm. During the centralized training, we assume the learning algorithm has access to all agents' individual observation-action histories and global state $s$. During the decentralized execution, each agent acts based on its learned action-value function $Q_i(\tau_i, a_i, m_i^{in})$ conditioning on its local action-observation history $\tau_i$ and received messages $m_i^{in}$. Message communication is also centrally learned and executed in a decentralized manner.

To solve this problem, we propose nearly decomposable value function. In our learning framework, individual action-value functions condition on local action-observation history and, at certain timesteps, messages from few other agents. We learn such near decomposable structure via learning minimized communication. We thus expect the communication to have the following properties:

\textbf{i) Expressiveness:} The message passed to one agent should effectively reduce the uncertainty in its action-value function.

\textbf{ii) Succinctness:} Agents are expected to send messages as short as possible to the agents who need it and when necessary.

To learn such a communicating strategy, we draw inspiration from variational inference for its proven ability in learning structure from data and endow a stochastic latent message space, which we also refer to as "message embedding". Messages are encoded as multi-variate Gaussian distributions with diagonal covariance in this latent space. Specifically, an encoder $f_m(m_i|\tau_i;\bm{\theta}_c)$ conditions on individual observation-action history is learned and shared among agents. At each timestep, this encoder outputs a message distribution $M_i$ for each agent $i$, from which a message $m_i^t$ is resampled. We adopt a point-to-point communication paradigm and $m_i^t=\langle m_{i1}^t, m_{i2}^t, ..., m_{in}^t\rangle$ where message $m_{ij}$, sampled from the distribution $M_{ij}$, is the message intended from agent $i$ to agent $j$. 

We impose constraints, which will be discussed in detail in the next section, on the latent message embedding to enable agent deciding locally which bits in a message should be sent (from 0 to all) according to their utility in terms of helping other agents make decision. Agent $j$ will receive an input message $m_j^{in}$ that has been cut, on which it conditions the local action-value function $Q_j(\tau_j, a_j, m_j^{in})$. All the individual Q values are then feed into a mixing network such as in QMIX~\citep{rashid2018qmix}.

Apart from the constraints on the message embedding, all the components (individual action-value function, message encoder, and mixing network) are trained end-to-end by the downstream TD loss. Thus, our overall objective is minimize
\begin{eqaution}
    \mathcal{L}(\theta) = \mathcal{L}_{TD}(\theta) + \mathcal{L}_c(\bm{\theta}_c),
\end{eqaution}
where $\mathcal{L}_{TD} = (r + \gamma \max_{a'} Q_{tot}(s', \bm{a'}; \theta^-)- Q_{tot}(s, \bm{a}); \theta)^2$ ($\theta^-$ are the parameters of a target network as in DQN) is the TD loss and $\theta$ is all the parameters in the model. We now discuss how to get $\mathcal{L}_c(\bm{\theta}_c)$ to regularize the message embedding.

\subsection{Minimized Communication Objective and Variational Bound}

Introducing a latent variable facilitates the representation of message, but it does not mean that the messages can reduce uncertainty in action-value functions of other agents. To achieve this goal, we maximize the mutual information between message $M_{ij}$ and optimal action policy of agent $j$, $A_j$, $I_{\bm{\theta}_c}(A_j; M_{ij} | \Tau_j, M_{(\shortn i)j})$. However, if this is the only objective, the encoder can easily learn to cheat by giving messages under different histories a representation in different regions in the latent space, rendering cutting off useless message difficult. A natural constraint to avoid such representation is the entropy of the messages. Therefore, our objective for message of agent $i$ is to maximize:
\begin{equation}\label{equ:original_objective}
    J_{\bm{\theta}_c}[M_i | \Tau_j, M_{(\shortn i)j}] = \sum_{j=1}^n I_{\bm{\theta}_c}(A_j; M_{ij} | \Tau_j, M_{(\shortn i)j}) - \beta H_{\bm{\theta}_c}(M_{ij}),
\end{equation}

where $\beta$ is a scaling factor trading expressiveness and succinctness and $M_{ij}$ is the message distribution intended from $i$ to $j$.

This objective is appealing because it agree exactly with the desiderata that we impose on the message embedding. However, applying this objective to our message embedding needs extra efforts because mutual information and entropy becomes intractable. By introducing a variational approximator, a popular technique from variational toolkit~\citep{alemi2017deep}, we can construct a lower bound on the mutual information term in Eq.~\ref{equ:original_objective}:
\begin{equation}\label{equ:mi_lower_bound}
\begin{aligned}
    & I_{\bm{\theta}_c}(A_j; M_{ij} | \Tau_j, M_{(\shortn i)j}) \\
& \ \ge  \ \mathbb{E}_{\bm{\Tau} \sim \mathcal{D}, M_{j}^{in} \sim f_m(\bm{\Tau};\bm{\theta}_c)} \left[ -\mathcal{CE}\left[ p(A_j | \bm{\Tau}) \Vert q_{\xi} (A_j | \Tau_j, M_{j}^{in}) \right] \right],
\end{aligned}
\end{equation}

where $\Tau_j$ is local action-observation history of agent $j$ and $\bm{\Tau}=\langle\Tau_1, \Tau_2, \dots,\Tau_n\rangle$ is the joint local history sampled from the replay buffer $\mathcal{D}$, $q_{\xi} (A_j | \Tau_j, M_{j}^{in})$ is the variational posterior estimator with parameters $\xi$. $\mathcal{CE}$ is the cross entropy. We share $\xi$ among agents to accelerate learning.

Next we discuss how to minimize the term $\beta H(M_{ij})$. Directly minimize the entropy of Gaussian distribution can cause the variance to collapse to 0. To deal with this possible numeric issue, we set the covariance to unit matrix and minimize $H(M_{ij}) - H(M_{ij} | \Tau_i)$ instead,  where $\Tau_i$ is the random variable of local history of agent $i$. This is equivalent because $H(M_{ij} | \Tau_i)$ is a multivariate Gaussian random variable whose entropy is a constant ($\log(\det(2\pi e \bm\Sigma)) / 2$, where $\Sigma$ is the unit matrix). Then we have:
\begin{equation}
    H(M_{ij}) - H(M_{ij} | \Tau_i) = \int p(m_{ij} | \tau_i) p(\tau_i) \log\frac{p(m_{ij} | \tau_i)}{p(m_{ij})} dm_{ij} d\tau_i.
\end{equation}
We use the same technique as in the mutual information term -- introducing an variational inference distribution $r(m_{ij})$ to approximate $p(m_{ij})$, and we can get:
\begin{equation}\label{equ:entropy_lower_bound}
\begin{aligned}
    H(M_{ij}) - H(M_{ij} | \Tau_i) & \le \int p(m_{ij} | \tau_i) p(\tau_i) \log\frac{p(m_{ij} | \tau_i)}{r(m_{ij})} dm_{ij} d\tau_i \\
                                & =   \mathbb{E}_{\Tau_{i}\sim D}\left[ \KL(p(M_{ij} | \Tau_i) \Vert r(M_{ij})) \right].
\end{aligned}
\end{equation}
This bound holds for any distribution $r(M_{ij})$. To facilitate cutting off messages, we use unit Gaussian distribution $\mathcal{N}(0,\mathbf{I})$. Combining Eq.~\ref{equ:mi_lower_bound} and~\ref{equ:entropy_lower_bound}, we get a tractable variational lower bound of our objective in Eq.~\ref{equ:original_objective}:
\begin{equation}\label{equ:objective}
\begin{aligned}
    & J_{\bm{\theta}_c}[M_i | \Tau_j, M_{(\shortn i)j}] \\
    \ge & \ \mathbb{E}_{\bm{\Tau} \sim \mathcal{D}, M_{j}^{in} \sim f_m(\bm{\Tau};\bm{\theta}_c)} \left[ -\mathcal{CE}\left[ p(A_j | \bm{\Tau}) \Vert q_{\xi} (A_j | \Tau_j, M_{j}^{in}) \right] -\beta \KL(p(M_{ij} | \Tau_i) \Vert r(M_{ij})) \right].
\end{aligned}
\end{equation}
We optimize this bound to get a expressive and succinct message embedding. Specifically, we minimize:
\begin{equation}\label{equ:loss}
\begin{aligned}
    \mathcal{L}_c(\bm{\theta}_c) = 
    \mathbb{E}_{\bm{\Tau} \sim \mathcal{D}, M_{j}^{in} \sim f_m(\bm{\Tau};\bm{\theta}_c)} \left[ \mathcal{CE}\left[ p(A_j | \bm{\Tau}) \Vert q_{\xi} (A_j | \Tau_j, M_{j}^{in}) \right] +\beta \KL(p(M_{ij} | \Tau_i) \Vert r(M_{ij})) \right].
\end{aligned}
\end{equation}

Intuitively, the first term, which we call the expressiveness loss, guarantees that messages sent can reduce the uncertainty in action-value functions of other agents. The second term, called succinctness loss, forces messages to get close to unit Gaussian distribution. Since we set covariance of message embedding to unit matrix, this term actually pushes the mean of messages to the origin of the latent space. Use this two losses leading to an embedding where useless messages distributes all near the origin, while messages that can contains information important for decision processes of other agents occupy other spaces.

Our message encoder $f_m(M_i|\Tau_i; \bm{\theta}_c)$ is updated guided by two gradients: stochastic gradient given by Eq.~\ref{equ:objective} and the gradient associated with TD loss.

\subsection{Cutting Off Messages}
Our objective compresses messages which can not reduce the uncertainty in action-value functions of other agents to the origin of the latent message space. This naturally gives us a hint to drop out meaningless messages -- we can order the message distributions according to their means and drop accordingly. Note that since we adopt diagonal covariance for our message embedding, bits in a message are independent. We thus make decision bit by bit and send messages with various length. In this way, such method not only finds out when to communicate (agent keep silence when all bits are cut), but also what to send (how many bits are sent and their values). Implementation details are discussed in Appendix~\ref{appendix:implementation}.


% First, computing mutual information is computationally challenging -- messages are encoded as continuous multi-variate Gaussian random variable. And, secondly, directly minimizing the entropy of Gaussian random variable may cause its variance to collapse to zero, resulting in intractable numeric issue.


